Update on Heavy-Meson Spectrum Tests of the Oktay--Kronfeld Action

We present updated results of a numerical improvement test with heavy-meson spectrum for the Oktay--Kronfeld (OK) action. The OK action is an extension of the Fermilab improvement program for massive Wilson fermions including all dimension-six and some dimension-seven bilinear terms. Improvement terms are truncated by HQET power counting at $\mathrm{O}(\Lambda^3/m_Q^3)$ for heavy-light systems, and by NRQCD power counting at $\mathrm{O}(v^6)$ for quarkonium. They suffice for tree-level matching to QCD to the given order in the power-counting schemes. To assess the improvement, we generate new data with the OK and Fermilab action that covers both charm and bottom quark mass regions on a MILC coarse $(a \approx 0.12~\text{fm})$ $2+1$ flavor, asqtad-staggered ensemble. We update the analyses of the inconsistency quantity and the hyperfine splittings for the rest and kinetic masses. With one exception, the results clearly show that the OK action significantly reduces heavy-quark discretization effects in the meson spectrum. The exception is the hyperfine splitting of the heavy-light system near the $B_s$ meson mass, where statistics are too low to draw a firm conclusion, despite promising results.

==> Makefile <==
DRIVE = ./.cloud/

MAKE := Makefile
#---------------------------------------------------------------------

TEXS := $(wildcard *.tex tables/*.tex)
MAIN := main.tex
BIB	 := refs.bib

PDF_FIG := $(wildcard ./figs/*.pdf)

AUX = $(wildcard *.aux *.log *.nav *.out *.snm\
				*.toc *.vrb *.blg *.dvi *.lof *.lot)

BBL := $(wildcard *.bbl)
STY := $(wildcard PoS*)

TARGET = $(MAIN:%.tex=%.pdf)

#---------------------------------------------------------------------

LATEX := latex
PDFLATEX := pdflatex

#---------------------------------------------------------------------

build : $(TARGET)
	make tmpclean

all : build

debug : $(TARGET)

cloud : build
	cp -a $(TARGET) $(DRIVE)

tmpclean:
	@rm -f $(AUX)

clean:
	@rm -f $(AUX) $(BBL) $(TARGET) *~

%.pdf : %.tex $(MAIN) $(TEXS) $(BIB) $(PDF_FIG) $(MAKE)
	$(PDFLATEX) $(basename $<)
	bibtex      $(basename $<)
	$(PDFLATEX) $(basename $<)
	$(PDFLATEX) $(basename $<)
	$(PDFLATEX) $(basename $<)

tar :
	tar -czf paper.tar.gz $(TEXS) $(PDF_FIG) $(BBL) $(STY)

